The Fate of Dwarf Galaxies in Clusters and the Origin of Intracluster Stars

This thesis presents a review of related important concepts in cosmology followed by details of the author's role in a research project on the origin of intracluster light. The author's role in the development of the simulations varied from searching parameters in the literature, through writing and modifying code in IDL, FORTRAN, and UNIX to carrying out hundreds of simulations using the particle-particle algorithm described in this thesis, as well as partaking in joint analysis of the simulation results. Part of this work in the isolated cluster simulations has been submitted for publication (Barai, Brito & Martel 2009). The main results of the simulations described in this thesis are: 1) destruction of dwarf galaxies by mergers dominates destruction by tides, and 2) destruction of galaxies by tides is sufficient to explain the observed intracluster light. These results support the accepted explanation for the origin of the intracluster light. In an ongoing, second stage of the simulation, which extends the isolated cluster results to a cosmologically significant region of the Universe, the author similarly assists in the implementation of a particle-particle/particle-mesh simulation and the joint analysis of the results to-date. The results are as per the Schechter luminosity function, and suggest the approach used is valid and the results obtained robust.

==> deluxetable.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% deluxetable.sty:  Standalone definitions of aastex's deluxetable. 
% 
% Credit: This file kindly provided by Alexey Vikhlinin. 
% 
% USAGE: 
% 
% 1. Put \usepackage{deluxetable} in the preamble of your document. 
% 2. Copy this text to a local file called deluxetable.sty. 
% 
\NeedsTeXFormat{LaTeX2e}[1995/12/01]% 
\ProvidesPackage{deluxetable}% 

\newcommand\nodata{ ~$\cdots$~ }% 
\newcommand\ulap[1]{\vbox\@to\z@{{\vss#1}}}% 
\newcommand\dlap[1]{\vbox\@to\z@{{#1\vss}}}% 

\newcommand\let@environment[2]{% 
 \expandafter\let 
 \csname#1\expandafter\endcsname\csname#2\endcsname 
 \expandafter\let 
 \csname end#1\expandafter\endcsname\csname end#2\endcsname 
 }% 

\def\substitute@command#1#2{% 
 \ClassWarning{aastex}{% 
  Command \protect#1\space is deprecated in aastex. 
  Using \protect#2\space instead (please fix your document). 
 }% 
 #2% 
}% 
\def\remove@command#1{% 
 \ClassWarning{aastex}{% 
  Command \protect#1\space is deprecated in aastex. 
  Please remove it from your document% 
 }% 
}% 
\def\@provide#1{%Implicit #2 
 \@ifxundefined#1{\def#1}{\def\@tempa}% 
}% 
\def\prepdef#1#2{% 
 \@ifxundefined#1{\toks@{}}{\toks@\expandafter{#1}}% 
 \toks@ii{#2}% 
 \edef#1{\the\toks@ii\the\toks@}% 
}% 
\def\appdef#1#2{% 
 \@ifxundefined#1{\toks@{}}{\toks@\expandafter{#1}}% 
 \toks@ii{#2}% 
 \edef#1{\the\toks@\the\toks@ii}% 
}% 
\def\appgdef#1#2{% 
 \@ifxundefined#1{\toks@{}}{\toks@\expandafter{#1}}% 
 \toks@ii{#2}% 
 \xdef#1{\the\toks@\the\toks@ii}% 
}% 
\toksdef\toks@ii=\tw@ 
\long\def\@ifxundefined#1{\@ifx{\undefined#1}}% 
\def\@boolean#1#2{% 
  \long\def#1{% 
    #2% \if<something> 
      \expandafter\boolean@true 
    \else 
      \expandafter\boolean@false 
    \fi 
  }% 
}% 
\def\@boole@def#1#{\@boolean{#1}}% Implicit #2 
\@boole@def\@ifx#1{\ifx#1}% 
\@boole@def\@ifx@empty#1{\ifx\@empty#1}% 
\@boole@def\@ifnum#1{\ifnum#1}% 
\@boole@def\@ifdim#1{\ifdim#1}% 
\@boole@def\@ifvoid#1{\ifvoid#1}% 
\long\def\boolean@true#1#2{#1}% 
\long\def\boolean@false#1#2{#2}% 

\newcommand\tablenotemark[1]{% 
 \rlap{$^{\mathrm #1}$}% 
}% 
\def\@tablenotetext#1#2{% 
 \vspace{.5ex}% 
 {\noindent\llap{$^{#1}$}#2\par}% 
}% 
\def\@tablenotes#1{% 
 \par 
 \vspace{4.5ex}\footnoterule\vspace{.5ex}% 
 {\footnotesize#1}% 
}% 
\def\@tablenotes@pptt#1{% 
 \par 
 \vspace{3.2ex}\footnoterule\vspace{.4ex}% 
 {\footnotesize#1}% 
}% 
\AtBeginDocument{% 
 \let\tblnote@list\@empty 
}% 
\newcommand\tablenotetext[2]{% 
 \appgdef\tblnote@list{\@tablenotetext{#1}{#2}}% 
}% 
\def\spew@tblnotes{% 
 \@ifx@empty\tblnote@list{}{% 
  \@tablenotes{\tblnote@list}% 
  \global\let\tblnote@list\@empty 
 }% 
}% 
\prepdef\endtable{\spew@tblnotes}% 
\expandafter\prepdef\csname endtable*\endcsname{\spew@tblnotes}% 
\let\tableline=\hline 
\long\def\@makecaption#1#2{\vskip 2ex\noindent#1\ #2\par}% 
\newcommand\tablenum[1]{% 
 \def\thetable{#1}% 
 \let\@currentlabel\thetable 
 \addtocounter{table}{\m@ne}% 
}% 
\newcommand\dummytable{\refstepcounter{table}}% 
\newbox\pt@box 
\newdimen\pt@width 
\newcount\pt@line 
\newcount\pt@column 
\newcount\pt@nlines 
\newcount\pt@ncol 
\newcount\pt@page 
\newcommand\colhead[1]{\multicolumn{1}{c}{#1}\pt@addcol}% 
\newcommand\tabletypesize[1]{\def\pt@typesize{#1}}%AO-access to different type sizes in deluxetable 
\def\pt@typesize{}% 
\newcommand\tablecolumns[1]{% 
 \pt@column=#1\relax 
 \pt@ncol=#1\relax 
 \global\let\pt@addcol\@empty 
}% 
\newcommand\tablecaption[1]{\gdef\pt@caption{#1}}% 
\newcommand\tablehead[1]{% 
 \gdef\pt@head{% 
  \hline\hline 
  \relax\\[-1.7ex]% 
  #1\hskip\tabcolsep 
  \\[.7ex]% 
  \hline 
  \relax\\[-1.5ex]% 
 }% 
}% 
\def\tablehead@aj#1{% 
 \gdef\pt@head{% 
  #1\hskip\tabcolsep 
  \\[.7ex]% 
  \hline 
  \relax\\[-1.5ex]% 
 }% 
}% 
\newif\if@pt@rot 
\newcommand\rotate{\@pt@rottrue}% 
\newcommand\tabletail[1]{\gdef\pt@tail{#1}}% 
\newcommand\tablewidth[1]{\pt@width=#1\relax}% 
\newcommand\tableheadfrac[1]{\gdef\pt@headfrac{#1}}% 
\AtBeginDocument{% 
 \let\pt@caption\@empty 
 \let\pt@head\@empty 
 \let\pt@tail\@empty 
 \pt@width\textwidth 
 \def\pt@headfrac{.1}% 
}% 
\def\pt@calcnlines{% 
 \begingroup 
  \if@pt@rot\textheight\textwidth\fi 
  \pt@typesize%AO-type sizes in deluxetable 
  \@tempdima\pt@headfrac\textheight 
  \@tempdimb\textheight\advance\@tempdimb by-\@tempdima 
  \@tempdima\arraystretch\baselineskip 
  \divide\@tempdimb by\@tempdima 
  \global\pt@nlines\@tempdimb 
 \endgroup 
}% 
\def\pt@tabacol{% 
 \edef\@preamble{\@preamble\hskip\tabcolsep\tabskip\fill}% 
}% 
\newdimen\pt@tmpcapwidth 
\long\def\@makecaption@plano#1#2{% 
 \@ifdim{\pt@width>\z@}{% 
  \pt@tmpcapwidth\pt@width 
 }{% 
  \pt@tmpcapwidth\textwidth 
 }% 
 \center 
  \parbox{\pt@tmpcapwidth}{% 
   \@make@caption@text{#1}{#2}% 
  }% 
 \endcenter 
}% 
\def\fnum@ptable{Table \thetable}% 
\def\fnum@ptablecont{Table \thetable \,\,  {\rmfamily (cont'd)}}% 
\long\def\@make@caption@text#1#2{% 
 \center\rmfamily#1.\quad#2\endcenter 
}% 
\long\def\@makecaption@plano@cont#1#2{% 
 \center\rmfamily#1\endcenter 
 \vskip 2.5ex 
}% 
\def\fnum@ptablecont@pptt{Table \thetable \,\,  {\itshape (cont'd)}}% 
\long\def\@make@caption@text@pptt#1#2{% 
 \center\sc#1\\[.5ex]#2\endcenter 
}% 
\long\def\@makecaption@plano@cont@pptt#1#2{% 
 \center\sc#1\endcenter 
 \vskip 1.5ex 
}% 
\def\fnum@ptable@apj{TABLE \thetable}% 
\def\fnum@ptablecont@apj{TABLE \thetable \,\,  {\itshape (cont'd)}}% 
\long\def\@make@caption@text@apj#1#2{% 
 \center\Large\sc#1\\[.5ex]#2\endcenter 
}% 
\long\def\@makecaption@plano@cont@apj#1#2{% 
 \center\Large\sc#1\endcenter 
 \vskip 1.5ex 
}% 
\def\fnum@ptable@aj{Table \thetable.}% 
\def\fnum@ptablecont@aj{Table \thetable.\space{\rmfamily (continued)}}% 
\long\def\@make@caption@text@aj#1#2{% 
 \center\large{\sc#1}\space#2\endcenter 
}% 
\long\def\@makecaption@plano@cont@aj#1#2{% 
 \center\large{\sc#1}\endcenter 
 \vskip 1.5ex 
}% 
\newenvironment{deluxetable}[1]{% 
 \def\pt@format{\string#1}% 
 \let\@acol\pt@tabacol 
 \let\@tabularcr\@ptabularcr 
 \let\@tablenotetext\@ptablenotetext 
 \let\@tablenotes\@ptablenotes 
 \global\pt@ncol\z@ 
 \global\pt@column\z@ 
 \global\pt@page\@ne 
 \gdef\pt@addcol{\global\advance\pt@ncol\@ne}% 
}{% 
 \spew@tblnotes 
 \typeout@deluxetable 
 \endcenter 
 \end@plano@float 
}% 
\let@environment{planotable}{deluxetable}% 
\def\@plano@float{% Invoked by \startdata 
 \begingroup 
  \if@pt@rot\columnwidth\textheight\fi %AO-deluxetable \rotate 
  \@plano@float@{table}% 
}% 
\def\end@plano@float{% S/B invoked by \enddata; instead by \enddeluxetable 
  \end@plano@float@ 
 \endgroup 
}% 
\def\@plano@float@{\@float}%AO-extra layer of abstraction for float processing 
\def\end@plano@float@{\end@float}% 
\appdef\@endfloatbox{% 
 \if@pt@rot\global\setbox\@currbox\vbox{\rotatebox{90}{\box\@currbox}}\fi 
}% 
\def\typeout@deluxetable@mss{% 
 \typeout{% 
  Table \thetable\space has been set to width \the\pt@width 
 }% 
}% 
\def\typeout@deluxetable@ppt{% 
 \typeout{% 
  Page  \the\pt@page \space of table \thetable\space has been set to 
  width \the\pt@width\space with \the\pt@nlines\space lines per page 
 }% 
}% 
\let\typeout@deluxetable\typeout@deluxetable@mss 
\newcommand\startdata{% 
 \pt@calcnlines 
 \@ifdim{\pt@width>\z@}{% 
  \def\@halignto{\@to\pt@width}% 
 }{% 
  \def\@halignto{}% 
 }% 
 \let\fnum@table=\fnum@ptable 
 \let\@makecaption\@makecaption@plano 
 \global\pt@line\z@ 
 \start@pt@tabular 
 \after@startdata 
}% 
\def\start@pt@tabular{% 
 \@plano@float 
 \center 
 \expandafter\caption\expandafter{\pt@caption}% 
 \pt@typesize%AO-type sizes in deluxetable 
 \expandafter\@tabular\expandafter{\pt@format}% 
}% 
\def\set@pt@box#1{\setbox\pt@box}% 
\def\after@startdata{\pt@head}% 
\def\after@startdata@aj{\hline\hline\relax\\[-1.7ex]\pt@head}% 
\def\enddata{% 
 \crcr 
 \noalign{\vskip .7ex}% 
 \before@enddata 
 \endtabular 
 \setbox\pt@box\lastbox 
 \pt@width\wd\pt@box\box\pt@box 
}% 
\def\before@enddata{\hline}% 
\def\before@enddata@aj{\hline\hline}% 
\def\nl{\substitute@command\nl\\}% 
\def\nextline{\substitute@command\nextline\\}% 
\def\@ptabularcr{% 
 {\ifnum0=`}\fi % A klootch just in case the next token is & or \cr 
 \@ifstar{% 
  \@testopt{\@argptabularcr\@empty}\z@skip 
 }{% 
  \@testopt{\@argptabularcr\ptable@@split}\z@skip 
 }% 
}% 
\def\@argptabularcr#1[#2]{% 
 \ifnum0=`{\fi}% To undo the effect of the klootch. 
 \@ifdim{#2>\z@}{% 
  \unskip\@xargarraycr{#2}% 
 }{% 
  \@yargarraycr{#2}% 
 }\ptable@split#1% 
}% 
\def\ptable@split#1{% 
 \noalign{% 
  \global\advance\pt@line\@ne 
  \@ifnum{\pt@line<\pt@nlines}{}{% 
   \aftergroup#1% 
  }% 
 }% 
}% 
\def\ptable@@split{% 
  \before@suspendpt 
  \endtabular 
  \setbox\pt@box\lastbox 
  \pt@width\wd\pt@box\box\pt@box 
  \typeout@pt@nl 
  \global\advance\pt@page\@ne 
  \endcenter 
  \end@plano@float 
  \clearpage 
  \addtocounter{table}{\m@ne}% 
  \let\fnum@table=\fnum@ptablecont 
  \let\@makecaption\@makecaption@plano@cont 
  \global\pt@ncol=\pt@column%  Either 0 or value of \tablecolumns 
  \global\pt@line\z@ 
  \start@pt@tabular 
  \before@resumept 
  \pt@head 
}% 
\def\before@suspendpt{}% 
\def\before@resumept{}% 
\def\before@suspendpt@aj{\@tabularcr\noalign{\vskip .7ex}\hline}% 
\def\before@resumept@aj{\hline\relax\@tabularcr[-1.7ex]}% 
\def\typeout@pt@nl@ppt{% 
 \typeout{% 
  Page \the\pt@page\space of table \thetable\space has been set to 
  width \the\pt@width 
 }% 
}% 
\def\typeout@pt@nl@mss{% 
 \typeout{% 
  Page \the\pt@page\space of table \thetable\space has been set to 
  width \the\pt@width\space with \the\pt@nlines\space lines per page 
 }% 
}% 
\def\typeout@pt@nl@aj{% 
 \typeout{% 
  Table \thetable\space has been set to 
  width \the\pt@width\space with \the\pt@nlines\space lines per page 
 }% 
}% 
\let\typeout@pt@nl\typeout@pt@nl@mss 
\newcommand\tablevspace[1]{\substitute@command\tablevspace\\[#1]}% 
\newcommand\tablebreak{\substitute@command\tablebreak\\}%{\cr\ptable@@split}% 
\newcommand\cutinhead[1]{% 
 \noalign{\vskip 1.5ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -4ex}% 
 \multicolumn{\pt@ncol}{c}{#1}% 
 \@ptabularcr 
 \noalign{\vskip .8ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -2ex}% 
}% 
\def\cutinhead@ppt#1{% 
 \noalign{\vskip 1.5ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -2ex}% Style Note: in apj, it is -1.5ex 
 \multicolumn{\pt@ncol}{c}{#1}% 
 \@ptabularcr 
 \noalign{\vskip .8ex}% 
 \hline 
 \@ptabularcr 
 \noalign{\vskip -2ex}% 
}% 
\newcommand\sidehead[1]{% 
 \noalign{\vskip 1.5ex}% 
 \multicolumn{\pt@ncol}{@{\hskip\z@}l}{#1}% 
 \@ptabularcr 
 \noalign{\vskip .5ex}% 
}% 
\def\@ptablenotetext#1#2{% 
 \vspace{0ex}% Style Note: in ppt, it is gone 
 {\parbox{\pt@width}{\hskip1em$^{\mathrm#1}$#2}\par}% 
}% 
\def\@ptablenotes#1{% 
 \par 
 \vspace{2ex}% 
 {\setlength\parskip{1.5ex}#1}% 
}% 
\def\@ptablenotes@apj#1{% 
 \par 
 \vspace{2ex}% 
 {#1}% 
}% 
\newcommand\tablerefs[1]{\appgdef\tblnote@list{\@tableref{#1}}}% 
\def\@tableref#1{% 
 \par 
 \vspace*{3ex}% 
 {\parbox{\pt@width}{\hskip1em\rmfamily References. --- #1}\par}% 
}% 
\newcommand\tablecomments[1]{\appgdef\tblnote@list{\@tablecom{#1}}}% 
\def\@tablecom#1{% 
 \par 
 \vspace*{3ex}% 
 {\parbox{\pt@width}{\hskip1em\rmfamily Note. --- #1}\par}% 
}% 
\def\@tableref@pptt#1{% 
 \par 
 \vspace*{3ex}{% 
 \parbox{\pt@width}{\hskip1em{\sc References.---}#1}\par}% 
}% 
\def\@tablecom@pptt#1{% 
 \vspace*{3ex}{% 
 \parbox{\pt@width}{\hskip1em{\sc Note.---}#1}\par}% 
}% 
\endinput 
%% 
%% ................................... End of file `deluxetable.sty'.
